Detection and estimation of spacecraft maneuvers for catalog maintenance

Building and maintaining a catalog of resident space objects involves several tasks, ranging from observations to data analysis. Once acquired, the knowledge of a space object needs to be updated following a dedicated observing schedule. Dynamics mismodeling and unknown maneuvers can alter the catalog's accuracy, resulting in uncorrelated observations originating from the same object. Starting from two independent orbits, this work presents a novel approach to detect and estimate maneuvers of resident space objects, which allows for correlation recovery. The estimation is performed with successive convex optimization without a-priori assumption on the thrust arcs structure and thrust direction.

==> Maneuver Detection Arxiv version/preamble.tex <==
% --------------- PREAMBLE / FLOAT ----------------

% floats
\usepackage{float}	 											% [H] positioning for tables
\usepackage[position=bottom,
			font=footnotesize,
		 	skip=0pt]{subcaption}								% \subcaptionbox labelled subfigures
	\renewcommand\thesubfigure{(\alph{subfigure})} 			 	% [1] set \autoref, \cref output to 'Figure 1(a)' style 
	\captionsetup[subfigure]{labelformat=simple}			 	% [2]

% spacing
\usepackage{setspace} 											% for local baseline skip control
\usepackage{caption}											% set space between floats and caption
	\captionsetup[table]{skip=5pt}
	\captionsetup[figure]{skip=8pt}

% set lengths			
\newcommand\newl[2]{ 											% shorthand for \newlength{\var}\setlength{\var}{x}
 	\expandafter\newlength\csname #1\endcsname
 	\expandafter\setlength\csname #1\endcsname{#2}}
\newcommand\setl[2]{ 											% renew option for lengths
 	\expandafter\setlength\csname #1\endcsname{#2}}

% initialise formatting lengths 
\newl{figh}{.0\columnwidth}										% picture height
\newl{figw}{.0\columnwidth}										% picture width
\newl{boxh}{.0\columnwidth}										% ecnlosing box height
\newl{boxw}{.0\columnwidth}										% ecnlosing box width
\newl{tcw}{.0\columnwidth}										% table column width

\newl{subfigskip}{.6em}											% subcaption-to-picture skip
\newl{plotvsep}{.8em}											% \vspace between vertically stacked pgf plots

% ---------------- PREAMBLE / TIKZ ----------------

% packages
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{positioning}

% general package settings
\pgfplotsset{
	compat=newest,
	plot coordinates/math parser=false,
}

% picture layers
\pgfdeclarelayer{annotation}
\pgfdeclarelayer{grid}
	\pgfsetlayers{grid,main,annotation}
% alignment grid
\newcommand{\addimagegrid}{1}									% ON/OFF switch for alignmend grid
\newcommand{\imagegrid}{										% grid style
	\begin{pgfonlayer}{grid}
		\draw[black!5, ultra thin, step=1,] (img.south west) grid (img.north east);
	 	\draw[black!15, ultra thin, step=10,] (img.south west) grid (img.north east);
	 	\foreach \x in {0,10,...,100} { \node [below] at (\x,0) {\x};}
	 	\foreach \y in {0,10,...,100} { \node [left] at (0,\y) {\y};}
	\end{pgfonlayer}
}		


==> preamble.tex <==
% --------------- PREAMBLE / FLOAT ----------------

% floats
\usepackage{float}	 											% [H] positioning for tables
\usepackage[position=bottom,
			font=footnotesize,
		 	skip=0pt]{subcaption}								% \subcaptionbox labelled subfigures
	\renewcommand\thesubfigure{(\alph{subfigure})} 			 	% [1] set \autoref, \cref output to 'Figure 1(a)' style 
	\captionsetup[subfigure]{labelformat=simple}			 	% [2]

% spacing
\usepackage{setspace} 											% for local baseline skip control
\usepackage{caption}											% set space between floats and caption
	\captionsetup[table]{skip=5pt}
	\captionsetup[figure]{skip=8pt}

% set lengths			
\newcommand\newl[2]{ 											% shorthand for \newlength{\var}\setlength{\var}{x}
 	\expandafter\newlength\csname #1\endcsname
 	\expandafter\setlength\csname #1\endcsname{#2}}
\newcommand\setl[2]{ 											% renew option for lengths
 	\expandafter\setlength\csname #1\endcsname{#2}}

% initialise formatting lengths 
\newl{figh}{.0\columnwidth}										% picture height
\newl{figw}{.0\columnwidth}										% picture width
\newl{boxh}{.0\columnwidth}										% ecnlosing box height
\newl{boxw}{.0\columnwidth}										% ecnlosing box width
\newl{tcw}{.0\columnwidth}										% table column width

\newl{subfigskip}{.6em}											% subcaption-to-picture skip
\newl{plotvsep}{.8em}											% \vspace between vertically stacked pgf plots

% ---------------- PREAMBLE / TIKZ ----------------

% packages
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{positioning}

% general package settings
\pgfplotsset{
	compat=newest,
	plot coordinates/math parser=false,
}

% picture layers
\pgfdeclarelayer{annotation}
\pgfdeclarelayer{grid}
	\pgfsetlayers{grid,main,annotation}
% alignment grid
\newcommand{\addimagegrid}{1}									% ON/OFF switch for alignmend grid
\newcommand{\imagegrid}{										% grid style
	\begin{pgfonlayer}{grid}
		\draw[black!5, ultra thin, step=1,] (img.south west) grid (img.north east);
	 	\draw[black!15, ultra thin, step=10,] (img.south west) grid (img.north east);
	 	\foreach \x in {0,10,...,100} { \node [below] at (\x,0) {\x};}
	 	\foreach \y in {0,10,...,100} { \node [left] at (0,\y) {\y};}
	\end{pgfonlayer}
}		

